Distribution through Repeated Market with Buying Rights

Resource distribution is a fundamental problem in economic and policy design, particularly when demand and supply are not naturally aligned. Without regulation, wealthier individuals may monopolize this resource, leaving the needs of others unsatisfied. While centralized distribution can ensure fairer division, it can struggle to manage logistics efficiently, and adapt to changing conditions, often leading to shortages, surpluses, and bureaucratic inefficiencies. Building on previous research on market-based redistribution, we examine a repeated hybrid market that incorporates buying rights. These rights, distributed iteratively by a central authority (for instance, as digital tokens), are intended to enhance fairness in the system - a unit of right is required to acquire a unit of the resource, but the rights themselves can also be traded alongside the resource in the market. We analyze how this regulatory mechanism influences the distribution of the scarce resource in the hybrid market over time. Unlike past works that relied on empirical methods, we explore the exact analytical properties of a system in which traders optimize over multiple rounds. We identify its market equilibrium, which is a natural generalization of the free market equilibrium, and show that it is coalition-proof. To assess the fairness in the system, we use the concept of frustration, which measures the gap between the resources a buyer is entitled to through their buying rights and what they actually obtain through trading. Our main theoretical result shows that using buying rights reduces the frustration by at least half compared to the free market. Empirical evaluations further support our findings, suggesting the system performs well even beyond the theoretically studied assumptions.

==> _old_sections/01_intro.tex <==
\section{Introduction}
\label{sec.int}

% Distribution crises are extreme situations where the supply of a critically important good is so small that the actors realistically do not have the necessary minimum available to ensure function. Such situations have two basic characteristics from a distribution point of view:

% {\bf 1.} The {\em ethical fairness} of the distribution of supply of critical goods is important. According to the rules of fairness, which are declared in advance, it is possible to hypothetically distribute the supply of a critical commodity fairly among organizations.

% In other words, the buyers have {\em rights to purchase a fair amount} of the commodity in question. The total amount of rights to purchase the commodity  is equal to the amount of the commodity available on the market.

% {\bf 2.} The existence of a {\em market for a critical commodity} is the second essential aspect of the distribution. Lack of a critically important good leads to a significant increase in price, organizations try to obtain more than a fair amount to cover their needs, and this is always at the expense of other participants. 
% %A free market leads to a narrowing of distribution.

% {\em Since the flow of money and critical goods in a free market during
% a distribution crisis is mainly concentrated between sellers and active buyers, our aim is to extend the flow to passive buyers, in order to avoid situations where the distribution of scarce strategic material reaches only the most active.}

% \medskip

% Crises of distribution are situations where the availability of a vital resource severely limited. %that individuals or organizations are unable to acquire the minimum amount necessary for functioning. 
% These types of crises can occur due to a variety of reasons such as natural disasters, wars, or economic instabilities. From a distribution perspective, these situations possess two key characteristics that are important to consider.

% Firstly, the ethical fairness of the distribution of the scarce resource is crucial. During a crisis, the distribution of resources is often not equitable, with some individuals or organizations receiving a disproportionate amount of resources while others receive little to none. This is where the principle of fairness comes in, as it aims to ensure that the distribution of resources is as fair as possible, according to the rules of fairness, which are declared in advance. 
% \ml{Using these rules of fairness}, it is possible to hypothetically divide the limited supply fairly among different entities. In other words, buyers have the right to acquire a fair share of the commodity in question, and the total amount of rights to purchase the commodity is equal to the total amount available in the market. A central authority can then distribute the good in quantity equal to the right, which we consider an ideal benchmark \ml{feasible} allocation. This centralised approach however comes with economic and time-related inefficiencies~\cite{moroney1997relative}.


% \begin{figure}[h]
% \includegraphics[width=8cm]{Plot}
% \end{figure}
% \ml{The second key characteristics of distribution crises is the existence of a market for the critical resourse.} Markets, \ml{delete up to side} modeled as large single or double auctions with many sellers and buyers on each side, have the potential to distribute goods in a flexible and reliable manner~\cite{cripps2006efficiency}. %To improve the system's efficacy, the second important aspect of distribution crises is hence the presence of a market for the vital resource. 
% The downside of the free market is that in the absence of stable supply, the scarcity of the resource leads to a significant rise in prices, with organizations attempting to acquire more than their fair share, always at the expense of others. This can lead to a situation where the most powerful or well-connected individuals or organizations are able to acquire the majority of resources, leaving the less fortunate with little to no access to the vital resource. To prevent such scenarios, {\em our goal is to increase the flow of the resource} to more buyers, rather than allowing the distribution of scarce resources to be concentrated among the most active participants in the market. 

%This can be achieved by creating a market for the resource, where buyers can purchase the resource at a fair price by implementing a rationing system where resources are traded based on pre-established rules of fairness.

% In summary, distribution crises are extreme situations where the availability of a vital resource is limited, and it is important to consider the ethical fairness of the distribution in the presence of a market and \ml{to design a hybrid distribution system where autonomous behaviour of traders following their individual incentives leads to more fair distribution of resources than the free market.} Such approach may be thought of as analogous to the basic strategy of \cite{DKA}, which, however, studies a different problem, namely maximizing the potential of the marketplace to serve a re-distributive purpose.

Crises of distribution are situations where the availability of a vital resource is severely limited. These types of crises can occur due to a variety of reasons such as natural disasters, wars, or economic instabilities. There exists many mechanisms that may be deployed to distribute the resources in such situations, and as extreme opposites we consider two: a centralized distribution handled a delegated authority, and a fully decentralized distribution implemented by a market free of any interventions. 

Markets have the potential to distribute goods in a flexible and reliable manner among many buyers and sellers~\cite{cripps2006efficiency}. The downside of the free market is that in the absence of stable supply, the scarcity of the resource can lead to a significant rise in prices, with some traders attempting to acquire more than their \enquote{fair} share, always at the expense of others. This leads to a situation where the most powerful or well-connected individuals or organizations are able to acquire the majority of resources, leaving the less fortunate with little to no access to the vital resource. On the other hand, when the distribution is delegated to centralized authorities, the resources may be divided more fairly, in accordance with some pre-established well-behaved \enquote{rules} associating each buyer with their share of the amount of resource available. Such distributions constitute ideal feasible allocations. This centralised approach however comes with economic and time-related inefficiencies~\cite{moroney1997relative}.

To combine the advantages of both approaches, we propose an iterative hybrid distribution system consisting of two stages. In each iteration, the central authority first fairly distributes buying rights among the buyers. Second, the rights are traded alongside the resource in a market. The rationale behind this design is to increase the flow of the resource to more buyers over time, rather than allowing the distribution of scarce resources to be concentrated among the wealthiest participants.

\subsection{Structure of the proposed hybrid system}
\label{sub.mi}
As we explained, our system consists of a sequence of interactions taking place sequentially over discrete time. For simplicity, we assume that there is only one commodity to be distributed. Each interaction, which we refer to as the \enquote{extended market}, consists of two stages:
\begin{enumerate}
\item The first stage exemplifies a \enquote{claim problem} as studied in axiomatic resource allocation literature~\cite{T}, where a finite amount must be divided among a set of agents whose claims exceed the available amount. In our case, the amount corresponds to the total of the critical commodity the sellers declare to the authority they intend to sell. The buyers then state their claims for the commodity. However, unlike the standard interpretation as in bankruptcy problems, where conflicting claims arise from legal debt, we interpret the claims as agents' \enquote{needs} for the critical resource. This motivates the authority to divide the amount into buying rights of the same quantity, rather than directly into portions of the commodity amount, and the system moves to the second stage. %   Based on this information, \ml{the fairness mechanism of the system} assigns buying rights in accordance with pre-agreed rules of fairness.

\item The second stage is a market where 2 types of goods are traded: the critical commodity, and the buying rights. The stage can be implemented by various market models, but one restriction should always hold: at the end of each extended market, each buyer must hold at least as many rights as they do of the commodity. All rights are eliminated at the end of each market, and the commodity the buyers acquire is consumed as per their claims. %\ml{In the next market, the rights are assigned again independently on the current market trading.}

\end{enumerate}
% (see Section \ref{sec.fair}) to each buyer a fair amount of {\em rights to purchase the commodity}.

% \jc{Meli bychom diskutovat tri typy incentiv: (1) obecne strategizacni predpoklady traderu: vzajemna racionalita, optimalizace ocekavany utility, (2) jejich utility, co popisuji, sebestrednost, unilateralni deviace, koluze a (3) strategicke tendence misreportovat (demandy, penize, utility apod.): zda se, ze obecna incentivni kompatibilita nebude mozna.}

To accentuate the fairness perspective prioritized during crises, we refer to the division rules used in the first stage of the extended market to distribute the buying rights as fairness mechanisms. Drawing from the bankruptcy problems, the division/fairness rules are to be agreed on in advance based on societal and ethical preferences. Our aim is then to minimize the role of the central authority (leaving not just deciding on the prices, but also storage, delivery, etc., on the traders) while increasing the equity in contrast to unregulated markets. The idea is to widen the flow of the critical commodity to even less wealthy buyers by letting them accumulate funds over trading rounds by selling their buying rights. 

% {\bf The social objective.} The proposed hybrid \ml{distribution system} aims to widen the flow of a critical commodity during a distribution crisis by allowing active buyers to purchase rights from hesitant, passive buyers. These saved funds can then be used by passive buyers to acquire the commodity in subsequent markets, as rights are recalculated and renewed before each market.

% \ml{Our aim is that the role of a central authority is minimised and the widening of the flow is a consequence of the market based on autonomous behaviour of the traders. The central authority does not give incentives, it only checks that the bought commodity is supported by the buying rights.}

In order to gauge the effectiveness of this iterative system, we introduce a welfare measure of \enquote{frustration} for individual buyers. Since the claims of some buyers are not satisfied in full, there are always some \enquote{frustrated} buyers. We focus on the buying rights as an expression of the system's social objective. 
% \ml{reviewer: why frustration is the right measure? ...in terms of frustration, which at a conceptual level seems reasonable though one could argue that it really captures the social objective.}
Specifically, for a single extended market, {\em frustration} is defined as the ratio $0\leq a/r\leq 1$, where $r$ represents the amount of rights assigned to a buyer $b$, and $a$ is the difference between $r$ and the actual amount of the commodity purchased by $b$, assuming this difference is non-negative. If the difference is negative, the frustration is defined as zero\footnote{It is worth noting that this concept of frustration applies not only in times of crises, but also during normal market conditions and in unrestricted free markets for the critical commodity. In normal times, assigned rights are bigger or equal to demand, and buyers are able to purchase all of the goods they desire, thus their frustration is zero.}. This notion of frustration is similar to the concept of \enquote{deprivation cost} discussed in the work of \cite{HPJ}. %We focus on frustration instead of on measures like social welfare, as we are more concerned with social inequality. 

% \jc{Meli bychom diskutovat tri typy incentiv: (1) obecne strategizacni predpoklady traderu: vzajemna racionalita, optimalizace ocekavany utility, (2) jejich utility, co popisuji, sebestrednost, unilateralni deviace, koluze a (3) strategicke tendence misreportovat (demandy, penize, utility apod.): zda se, ze obecna incentivni kompatibilita nebude mozna.}

We adopt standard assumptions about the traders' strategic capabilities. Their utilities are real-valued monotone bi-variate functions of money and the critical commodity defined more rigorously in later sections. The traders are mutually rational, self-interested and aim to maximize their expected utilities. We assume the distribution system is implemented as a certified portal where the history of trading provides indirect mechanisms for (checking) truthful reporting of buyers' claims. 
As the commodities flow through the portal only, the misreported claims provide the only avenue for the traders to influence the commodity distribution in their favor. Incentive compatibility appears unachievable in general, yet the information superiority of the central authority enables deploying standard anti-collusion barriers. Moreover, we assume the complete history of trading of rights is known and archived, and the particular fairness and market mechanisms are agnostic to traders' identities.

% Our ultimate goal is to demonstrate that, in a sequence of markets using this system, the frustration of each buyer is smaller than it would be in a free market. This can be achieved by increasing the 
% \enquote{willingness to pay} of frustrated buyers through the trading of assigned rights.
% The {\em willingness to pay} of a buyer $b$  associates, with a positive $x$, maximum amount $w_b(x)$ of money of the same utility as amount $x$ of the critical commodity.

% {\bf The Rules of Fairness.}
% \jc{proc je frustrace dobra mira ferovosti, vztah gini a frustrace, frustrace je "lokalni" PoA se SW}
% \ml{The rules of fairness are agreed on in advance based on societal and ethical preferences. Our strategic view is that the fairness mechanism cannot be used as a redistribution mechanism of wealth.}

% \ml{reviewer: - Completely ignores incentive issues in the fairness mechanism. 

% -It is in principle a strength to have a mechanism that works in conjunction with any specified fairness principle. However I wonder if it is realistic that this can be separated.}

% {\bf Incentives to participate in the system.}
% \ml{why traders want to participate?}

% {\bf Coalition and strategic manipulation proofness} To improve the robustness of the system against strategic manipulation from the side of the traders, we require that after each market of the sequence, for each buyer there is a check whether their amount of the critical commodity is at most as large as their amount of right. 
% We further require that the distribution system is implemented in a certified portal, where the history of trading provides indirect mechanisms for (checking) truthful reporting of demand and supply, the complete history of trading of right is known and archived, and the particular trading mechanisms are agnostic to the trader's identities. 

% The group which suffers by the introduction of the Right are the rich buyers. However, even if all choose to deviate and not buy Right, it will not increase their payoff. This is because the sellers will keep offering the same amount of Good and the price would keep increasing. The sellers do not want to join this coalition and only keep selling to the rich buyers, since it would require them to keep some Good for future Market, decreasing their utility.
% \ml{reviewer - Other limiting or unstated assumptions in setup (e.g., why no seller supply curve, or storage of good across time)

% Similarly ignores strategic trading behavior in operation of auctions for each market.}

% \ml{add here from non-myopic:
% The introduction of the Right negatively impacts rich buyers. Even if they all choose to deviate and not purchase the Right, their payoff will not increase. This is because the sellers will continue to offer the same amount of Good, resulting in a continuously increasing price. Additionally, sellers do not want to join a coalition that only sells to rich buyers, as it would require them to hold back Good for future Markets, reducing their utility.}

% {\bf Comparison with alternative ways to distribute rights.}

% \ml{reviewer: What are the reasons to believe approach here is better than other ways of using rights distributions one could invent?

% - The model assumes that it makes sense to define levels of supply and demand for sellers and buyers, resp., without reference to price. One could argue that the supply curve during a crisis is steep, but it seems extreme to assume it is completely vertical.

% - Why is it reasonable to allow rights to be saved across periods, but not goods? This could cause rights to be less valuable later, though as far as I can tell there is no provision in the fairness mechanism to account for this.
% }
% \todo[inline]{(D) Já nevim, jestli sem dávat willingness to pay. Nemůžeme prostě říct, že intuitivně ty peníze můžou použít a dostat tak víc zboží později?}

% The idea is that some (active) buyers want to buy more of the good right away, so according to the rules of the market, they can buy from hesitant (passive) buyers an amount of rights assigned to them. With this money saved, even these passive buyers can buy the commodity in next markets, because the rights are recalculated before each market, and thus renewed.


% We need to introduce some measures indicating how successful the proposed hybrid mechanism is towards our goal of widening the flow of the critical commodity in the time of a distribution crisis. 
% For a single market, we define the {\em frustration} of a buyer $b$ as the ratio $0\leq a/r\leq 1$ where $r$ is the amount of the rights potentially assigned to $b$ and $a$ is the difference between $r$ and the amount of the good purchased by $b$, if this is at least zero, and it is defined to be zero otherwise.
% We note that the notion of frustration extends to normal times without crises and to the unrestricted free market with the critical commodity. In normal times, the amount of assigned rights is equal to the demand and moreover $b$ can buy all the goods it demands. Hence, its frustration is zero. Our concept of {\em frustration} is somewhat similar to  the {\em deprivation cost} of \citeauthor{HPJ}.

% Our aim is to show that in a sequence of markets of our system, {\em the frustration of each buyer becomes smaller than it would be in the free market}. In order for that to happen it is needed that the frustrated buyers increase their {\em willingness to pay} (formally introduced in Definition \ref{def.ww}).  Our proposed mechanism changes the willingness to pay by trading the assigned rights.

% \subsection{Robustness to strategic manipulation}
% \label{sub.coal}



\subsection{Main contributions} 

% As we explained, we study trading in a system consisting of a sequence of markets combined with a fairness mechanism for allocating the rights designed to improve social good. In Section~\ref{sec: trading env}, we formally define our hybrid trading environment, fairness mechanisms and the measure of equity we employ to evaluate the system's fairness -- the frustration. Frustration later gives rise to the analog of the Price of Anarchy in the trading environment. Our aim is to examine how the Price of Anarchy evolves when buying rights are incorporated. All our results are agnostic to the fairness mechanism used to distribute the rights.
% Our primary contribution is a formal construction of a system that explicitly separates allocation of buying rights and trading of goods during a middle of a distribution crisis characterized by relatively stable, albeit small, supply and over-exceeding demand.
Our primary contribution is the development of a formal system  based on autonomous behaviour of the traders which increases the flow of the resource to more buyers in a sequence of trading interactions over discrete time during the midst of a distribution crisis characterized by a relatively stable but limited supply and an excessive demand.
Each interaction is modelled as an extended market which clearly distinguishes the fair allocation of buying rights and the trading of goods.

% \ml{We show that in our system, the equilibrium of the free market is moved towards the social objective of wider distribution, i.e., less frustration of buyers, by autonomous strategic behaviour of the traders.}

We investigate the impact of incorporating a fairness mechanism for allocating rights to purchase in a sequence of over-demanded markets. Specifically, we formalize our hybrid trading environment, including the fairness mechanisms and the measure of distribution effectiveness, defined as frustration, in Section~\ref{sec: trading env}. We then use this per-buyer frustration welfare measure to analyze the evolution of overall expected frustration in this environment with two different implementations of the single-round markets. To the best of our knowledge, we are the first to rigorously analyze a system explicitly combining a market mechanism with a fairness mechanism allocating buying rights for more socially just redistribution of critical goods during the times of need. It is important to note that our findings are independent of the specific fairness mechanism used.


In Section~\ref{sec:myopic}, we delve into the analysis of solutions in systems where traders are myopic, in the form of market-clearing prices with rights.  We formulate an auction-based algorithm that can approximate the solution in polynomial time while providing a guarantee on its quality.
\begin{cmr}{Theorem \ref{thm.mmain} (informal)}
There exists an algorithm with time complexity cubic in the number of traders that approximates the maximum clearing solutions of the extended market with myopic traders such that each trader receives a utility at least $(1-2\epsilon)$-times their optimum.
 \end{cmr}
 \noindent Using this result, we are able to bound the overall expected frustration in the system, showing that the equilibrium of the free market is moved towards the social objective of wider distribution.
 \begin{cmr}{Theorem \ref{thm.wp} (informal)}
Consider a sequence of extended markets where for each buyer the amount of available money is non decreasing. If solutions are computed using the algorithm from Theorem~\ref{thm.mmain}, then up the first market, the expected frustration is at most $1/2$.
\end{cmr}

Section~\ref{sec:nonmyopic} then considers a more complex system with traders who optimize over the entire crisis. We examine properties of the arising equilibrium and design an algorithm computing it efficiently.
\begin{cmr}{Theorem \ref{thm:greedy:equilibrial} (informal)}
There exists an algorithm with time complexity linear in the number of traders that computes a coalition-proof equilibrium of the system with non-myopic traders with linear utilities.
% The Greedy strategies \eqref{eq: seller policy} and \eqref{eq: buyer policy} form a coalition-proof equilibrium of a feasible Sequence of any length. The equilibrium can be computed efficiently.
\end{cmr}
Further analysis of the equilibrium reveals the equilibrium offers a similar asymptotic upper bound on the expected frustration as in the system with myopic traders.
\begin{cmr}{Theorem \ref{thm:nonmyopic:poa} (informal)}
% Consider a Sequence where traders follow the Greedy strategy. Then the Price of Anarchy in the Market with fairness is at most 1/2 of the free market's PoA as ${\cal T} \to \infty$.
Consider a sequence of extended markets where traders follow the equilibrial strategies from Theorem~\ref{thm:greedy:equilibrial}. Then the Price of Anarchy is at most $1/2$ as the number of markets tends to infinity. 
\end{cmr}

In the last part of the paper, we summarize the desired features of the trading system and provide several potential future directions. Due to space constraints, full versions of all proofs are in Appendix~\ref{app: proofs}. 
Complete analysis of the general system is out of our reach. However, we do make several encouraging observations.

% Our priority in this work is to study the behavior of a large complex system, which makes it difficult to analyze the traders' behavior theoretically. For this reason, in Section 4, we introduce a reinforced-learning algorithm in an attempt to approximate the system's equilibrium. In Section 5 we present the empirical results. First, we perform a thorough numerical analysis demonstrating how close to the equilibrium we are able to converge to. Then we carry out a series of ablation experiments, showing that the Price of Anarchy in the system without the fairness mechanism may be high.
% Then we perform a thorough numerical analysis of multiple settings of the system, varying the number of inner trading iterations and lengths of the sequence of markets.
% We confirm that together with intuitive governmental regulations akin to increased storing prices for the goods, the system with the fairness mechanism is able to decrease the Price of Anarchy. In the last part of the paper, we summarize the desired features of the trading system enlightened by the experiments.



% \todo {REWRITE AS LAST THING, not edited}
% XXXXXXXXXXXXX


% We consider the question of how to allocate a good that is over-demanded in a  multi-round scenario which we call a {\em distribution crisis}, in order to improve the fairness of the free market allocation. 

% This is by itself an important subject of economic interest. We believe that our construction, in particular introducing rights to purchase,
% separating rights and goods and trading them separately may be useful in other fairness contexts as well.

% A distribution crisis for a commodity which needs to be supplied regularly is typically preceded by significant changes in demand and/or supply, causing a sudden change of the market. Modelling these early stages is a growing research area [???], however typically requires non-trivial assumptions about the nature of the crisis. 

% Final rounds of a distribution crisis are also very complex to model and analyse since an optimal outcome of a participant for the terminal segment of a crisis does not necessarily decompose into his optimal outcomes in each round; the participants strategize when a termination of a crisis becomes apparent.

% We instead choose to model the middle of the multi-round distribution crisis, where the supply and demand is relatively stable and the participants aim the optimal outcome of each round. 

% A key new idea is, in each round, to trade separately allocated amount of Right and available amount of Good.  Agents who have the rights to an amount of Good but whose per-unit utility is low can sell their rights to others, raising funds to purchase Good in future rounds.

% XXXXXXXXXXX




%We further simplify by having only one type of scarce resource called {\it Good}. 



%Our multi-round trading environment, which we call {\em Crisis}, is formally introduced in Section \ref{sec.def}.

%First step in  is to have a benchmark "fair" allocation given the needs of the buyers and the supply of the suppliers. We go into more detail on what ``fair" means in Section \ref{sec.fair}.

%The second step of our solution is introduction of a trading environment which is meant to increase fair allocation of Good among buyers.  We accomplish this by introducing a new tradable commodity which we call {\it Right}: it represents right to buy Good and it is distributed in the beginning of each round according to the benchmark allocation. Without the Right, our solution reduces to the multi-round free market for the Good.

% \todo[inline]{(D) Až sem se mi zdá, že je to spíš problem definition než main contribution.}

%In Section \ref{sec.alg},\todo{(D) Tohle by asi měla být sekce 3, ne 3.1.} we describe a polynomial auction-based algorithm and show in Theorem \ref{thm.mmain} that for a practically non-restrictive choice of parameters it outputs an approximate optimal market clearing solution for the Crisis. 

%In the remaining part of the paper, starting with Theorem \ref{thm.wp},\todo{(D) je to spíš už od sekce \ref{s.wp}, kde se to na začátku píše ne?} we further assume that the amount of Good in each round as well as the utilities of traders are constant. This is a realistic assumption for the middle of a distribution crisis.


%Informally, an interaction between buyers and sellers is as follows. First, each seller offers some amount of Good he has for sale for some price. Based on the total offered volume of Good and the Demand of buyers, a central {\it fairness mechanism} then assigns buyers with Right. In the second stage, the buyers offer some amount of Right for sale for a fixed price. Given offers for both Right and Good, the buyers then declare maximum volume and price they are willing to pay for both. A {\it market mechanism} then clears the bids. 

% We show that the introduced mechanism approximates the fair benchmark allocation at an equilibrium of behavior.

% \todo[inline]{(D) V téhle části by se měly říct dvě věci: (1) stabilní situaci (tedy uprostřed krize) řešíme analyticky pro dva modely, které jdou efektivně implemntovat, protože pro ně je poly-time výpočet (2) pro oba vyjde PoA <= 1/2.}

% A way to measure exploitability of a mechanism is coalition proofness, that is the smallest coalition which can deviate from the proposed strategy and gain utility. In our setting, one group which is suffering compared to the free market are the rich buyers; thanks to buying right, they are acquiring less critical commodity. 
% \todo{(M) the idea is not clearly formulated} But even if {\it all} rich buyers decide to cooperate and \enquote{engage with the fairness}, the market doesn't change drastically. This is because the sellers will offer at most the volume they got in that market, ensuring the amount of right each buyer receives is the same. Without this, the rich buyers could over a long time increase the Right they would be getting to a point when they can buy Good with all Money they receive.
% It is not beneficial for a seller to join the coalition of the rich buyers to allow this scheme, since his utility would decrease by $c$ for each unit of Good he is keeping for the next Market.

% An appealing feature of our trading environment is that it is coalition proof with respect to the sellers. A natural attack of the system by the sellers, especially during a crisis, is to collectively increase the selling price of the critical commodity. However, as we have shown in Theorem \ref{thm.mmain} and in the proof of Theorem \ref{thm: equal prices}, the poor buyers would opt to sell their right at the same price, decreasing the profit of sellers since not all available critical commodity would be sold.


\subsection{Related work}

% \ml{reviewer: I think there is a better way to frame the problem in the paper. The “crisis” problem described in the paper appears to be closely related to the bankruptcy problem or the claims problem as studied in the axiomatic resource allocation literature (and discussed by William Thomson in his survey articles and books). The “frustration” language is quite appropriate in this setting. Agents start out with claims (what the paper calls “rights”) that add up to a total supply of a resource, which then gets partially destroyed (this is the crisis), thereby making the satisfaction of the claims impossible. The claims are frustrated.}

Allocating a set of resources to a set of individuals in a fair manner has been extensively studied over the past decades. The objective of a fair distribution is to identify an allocation mechanism that satisfies certain properties generally referred to as fairness criteria. In the literature, there is no clear definition of fairness, rather a wide variety of notions has been introduced; see for example \cite{far} for a survey. Many recent works considered the question of whether it is possible to simultaneously achieve fairness and efficiency, and studied Pareto optimality and fair allocations for various fairness notions. For example, \cite{CKM} presented inherent connection between Envy Freeness, Pareto optimality, and the notion of maximum Nash welfare. Our mechanism draws extensively from theory on claims and taxation problems, and primarily fair divisions in bankruptcy problems, a survey of which can be found in~\cite{T}.

Our work contributes to the field of redistributive mechanisms, particularly those aimed at reducing inequalities. A similar study in the literature examines a two-sided market trading goods of homogeneous quality, with the goal of optimizing the total utility of traders~\cite{DKA}. However, our approach differs in that we consider more general fairness measures, rather than just the social welfare, and assume that utilities are common knowledge. This work has been recently expanded to include a setting with heterogeneous quality of tradable objects, various measures of allocation optimality, and imperfect observations of traders~\cite{akbarpour2020redistributive}. Another related work examines multiple market and non-market mechanisms for allocating a limited number of identical goods to multiple buyers~\cite{condorelli2013market}. The author argues that when buyers' willingness to pay aligns with the designer's allocation preferences, market mechanisms are optimal, and vice versa. In crisis situations, it is reasonable to assume that critical resources are highly valuable to all participants, yet some may lack the money to acquire them. Combined with the fact that it is in society's best interest to allocate goods fairly, these findings suggest that relying solely on unregulated markets may not be the best approach in a distribution crisis.

Emissions allowances and tradable allowance markets present to a certain extent a similar mechanism to our work. Historically, tradable property rights were allocated by regulators directly to firms. This led to a number of inefficiencies, such as misallocation, regulatory distortions or barriers to entry the markets. Contemporary market designs utilize auctions for the allocation of tradable property rights. As presented in \cite{dor}, tradable allowance markets play an invaluable role in ensuring the efficiency of carbon markets and in the prevention of market power by large and dominant agents. In \cite{WCZ}, efficiency of multi-round trading auctions for allocation of carbon emission rights is studied. 

% \cite{ADG} develops a dynamic programming model for optimizing resource allocation by food banks among the agencies they serve. The framework measures effectiveness based on the nutritional value of the allocation decisions, efficiency as the utility of the agencies served, and equity as fairness in the allocation of food among those agencies. 


In our work, we differ from the existing related works by designing a trading-rationing mechanism that introduces rights to purchase a fair amount of the scarce commodity, allocates them in a fair manner and trades them together with the critical commodity in order to ensure that scarce resources can be allocated among agents in a fairer manner than by the free market.
To the extent of our knowledge, this is the first work that introduces such hybrid trading-rationing mechanism, and also analytically solves such a complex rationing scheme.




% Our work belongs to the literature on redistributive mechanisms, especially those mitigating inequalities. Perhaps the most related paper studies a two-sided market trading goods of homogeneous quality, optimizing the traders' total utilities~\cite{DKA}. The difference lies in our explicit incorporation of the buyers' varying needs into the consideration and the fact that in our model, the utilities are a common knowledge. This work was recently generalized into a setting with heterogeneous quality of tradable objects, more diverse measures of allocation optimality, and imperfect observations about the traders~\cite{akbarpour2020redistributive}. Another related work presents multiple markets and non-market mechanisms for allocating a limited number of identical goods to several buyers~\cite{condorelli2013market}. The author shows that when the buyers' willingness to pay coincides with the designer's allocation preferences, market mechanisms are optimal, and vice versa. In crises environments studied in our work, it is reasonable to assume that the critical resources are highly valuable to all participants, yet, some may lack the money to obtain them. Together with the fact that it is in society's best interests to allocate the goods fairly, these results suggest that leaving the distribution solely to unregulated markets is rather inadvisable. 






==> _old_sections/03_fairness.tex <==






==> _old_sections/05_fairness.tex <==
\section{Fairness}
\label{sec: fairness}
\todo{(D) Depricated, remove once unified.}

At the core of each Market defined in the previous Section is the fairness mechanism $\phi$, which assigns buyers Right to purchase Good. However, the notion of a ``fair" allocation is very subjective. As such, we try to restrict the mechanism as little as possible. As per Definition \ref{def: fairness mechanism}, we require that the fairness mechanism
\begin{enumerate}
    \item distributes Right for all offered Good;
    \item assigns no Right to buyers without Demand for the scarce resource;
    \item is non-decreasing with Demand of each buyer; and
    \item treats buyers with equal Demand equally.
\end{enumerate}
These conditions imply that the fairness function has a special ``distribution-induced" form
\begin{equation}
    \phi_b\left(\sum_{s\in S} v_s^\tau, D\right) = \alpha_b(D, V)\sum_{s\in S} v_s^\tau,
\end{equation}
where $\alpha$ is a distribution. Indeed, condition 1 implies $\sum_{b\in B}\alpha_b(D, V) = 1$ and conditions 2 \& 3 together imply $0 \le \alpha_b(D,V)\le 1$. The last condition restricts functional dependence of $\alpha$ on the Demand.

One example of the fairness mechanism is the {\it proportional fairness mechanism}, which allocates Right to $b$ proportionally to his Demand
\begin{equation}
    \phi_b\left(\sum_{s\in S} v_s^\tau, D\right) = \frac{D_b\sum_{s\in S} v_s^\tau}{\sum_{b\in B} D_b},
    \hspace{3ex}
    \alpha_b^\phi(D, V) = \frac{D_b}{\sum_{b\in B} D_b},
\end{equation}
where the distribution is not dependant on the total volume distributed.\todo{(D) It is the only such distribution, right?}

A class of fairness functions which will be of special importance is the {\it n-canonical fairness function} which allocates all Right to the buyer with the $n$-th highest Demand
\begin{equation}
    \varphi_{b, n}\left(\sum_{s\in S} v_s^\tau, D\right) = 
    \begin{cases}
    \sum_{s\in S} v_s^\tau & \text{if } D_b \text{ is the }n\text{-th highest Demand},\\
    0 & \text{otherwise}.
    \end{cases}
\end{equation}
where ties are broken arbitrarily but consistently.

\subsection{Frustration}
The Right can be thought of as the amount of Good a buyer is socially entitled to. In other words, if the distributional crisis is managed fully by a central authority, the buyer would receive that amount. A contrast between this ``most fair" centralized solution, and whatever a buyer is able to acquire is captured by his {\it frustration}.

Formally, the frustration of a buyer is normalized difference between the Right he would be assigned\footnote{We can also measure frustration in the free market, where no Right exists. However, a common notion of fair allocation may still exist.} and the amount of Good he acquired in a Market if that is at least zero, and zero otherwise. 
\begin{equation}
    f_b^\tau(\pi, G_T^\tau, M_T^\tau) = 
    \text{max}\left\{0, \frac{R_b^\tau - \mu^G_b(\pi, G_T^\tau, M_T^\tau, R^\tau)}{R_b^\tau}\right\},
\end{equation}
where $R^\tau = \phi(\sum_{s\in S} v_s^\tau, D)$.

\subsection{Price of Anarchy}
Consider now the point of view of the central authority, such as government of a country. As a result of trading the Good, the final allocation differs from distributing it centrally. This difference measures the inefficiency of the trading to allocate Good fairly. This is conceptually similar to the Price of Anarchy (PoA) [???], which measures the price the system pays for autonomous behaviour of the traders. As such, we define the Price of Anarchy in our system as scaled sum of frustrations of the buyers.
\begin{equation}
    PoA^\tau = \frac{\sum_{i=1}^\tau\sum_{b\in B}f_b^i}{\tau |B|}.
\end{equation}
Note that $PoA^\tau \ge 0$ since $f_b^\tau \ge 0$ and $PoA^\tau = 0 \Rightarrow f_b^i = 0 \ \forall b\in B, \forall i\in \{1,\dots \tau\}$. In the latter case, trading Good in the Market had the same social impact as distributing it centrally. 

We aim to show that, as a result of implementing Right, the Price of Anarchy decreases compared to the free market. Note that for the latter the PoA can be arbitrarily high if a buyer receives low amount of Money and has a high Demand.





==> _old_sections/07_buyer_driven_market.tex <==



==> _old_sections/fairness_universe.tex <==
\subsubsection{Universe of Fairness Distributions}
\label{sub.cg}
Let us assume we are dividing an estate $E$, and we assume $E$ is {\em divisible}. Let $d_1\leq \ldots \leq d_r$, $r= |B|$, be the demands of the buyers. Each fairness rule will be specified by two non-negative constants $c_1, c_2$ satisfying $c_1+ c_2 \leq 1$.
Let us think of the estate as gradually growing. 
\begin{enumerate}
    \item 
When it is small, all buyers divide it equally. This continues until buyer $1$ has received $c_1d_1$; for the time being she then stops receiving supplies, and the remaining supply is divided equally between the remaining $r-1$ buyers. This, in turn, continues until buyer $2$ has received $c_1d_2$, at which point she stops receiving supplies for the time being, and the remaining supply is divided equally between the remaining $r-2$ buyers. The process continues until each buyer has received $c_1$ of her claim. This happens when $E = c_1D$, where we let $D= \sum_{i=1}^rd_i$.
\item
When $E = c_1D$, the process continues proportionally until $E = (c_1+ c_2)D$.
\item
When $E = (c_1+ c_2)D$, the process is the mirror image of the first step above. Instead of thinking in terms of $i$'s award $x_i$, one thinks in terms of her loss $d_i-x_i$, the amount by which her award falls short of her demand. When the total loss $D- E$ is small, it is shared equally between all buyers. The buyers continue sharing total loss equally, until buyer $1$ has lost $(1- c_1- c_2)d_1$ (which is the same as receiving $(c_1+ c_2)d_1$). For the time being she then stops losing, and an additional total loss is divided equally between the remaining $r-1$ buyers. The process continues until each buyer has lost $(c_1+ c_2)$ of her demand, which happens when $E= (c_1+ c_2)D$. This is precisely to where we got in describing the first two parts of the procedure.
\end{enumerate}

We observe that (1) If $c_1= 1$, the resulting distribution is uniform, (2) If $c_2= 1$ then the resulting distribution is proportional, and (3) if $c_2$ is zero and $c_1$ is the half, then the resulting distribution is the contested garmet.

==> _old_sections/intro.tex <==
\section{Introduction}
\label{sec.int}

% Distribution crises are extreme situations where the supply of a critically important good is so small that the actors realistically do not have the necessary minimum available to ensure function. Such situations have two basic characteristics from a distribution point of view:

% {\bf 1.} The {\em ethical fairness} of the distribution of supply of critical goods is important. According to the rules of fairness, which are declared in advance, it is possible to hypothetically distribute the supply of a critical commodity fairly among organizations.

% In other words, the buyers have {\em rights to purchase a fair amount} of the commodity in question. The total amount of rights to purchase the commodity  is equal to the amount of the commodity available on the market.

% {\bf 2.} The existence of a {\em market for a critical commodity} is the second essential aspect of the distribution. Lack of a critically important good leads to a significant increase in price, organizations try to obtain more than a fair amount to cover their needs, and this is always at the expense of other participants. 
% %A free market leads to a narrowing of distribution.

% {\em Since the flow of money and critical goods in a free market during
% a distribution crisis is mainly concentrated between sellers and active buyers, our aim is to extend the flow to passive buyers, in order to avoid situations where the distribution of scarce strategic material reaches only the most active.}

% \medskip

Crises of distribution are situations where the availability of a vital resource is so limited that individuals or organizations are unable to acquire the minimum amount necessary for functioning. These types of crises can occur due to a variety of reasons such as natural disasters, wars, or economic instabilities. From a distribution perspective, these situations possess two key characteristics that are important to consider.

Firstly, the ethical fairness of the distribution of the scarce resource is crucial. During a crisis, the distribution of resources is often not equitable, with some individuals or organizations receiving a disproportionate amount of resources while others receive little to none. This is where the principle of fairness comes in, as it aims to ensure that the distribution of resources is as equitable as possible. According to the rules of fairness, which are declared in advance, it is possible to hypothetically divide the resource fairly among different entities. In other words, buyers have the right to acquire a fair share of the commodity in question, and the total amount of rights to purchase the commodity is equal to the total amount available in the market. A central authority can then distribute the good in quantity equal to the right. This centralised approach however comes with economic and time-related inefficiencies.

The second important aspect of distribution crises is the presence of a market for the vital resource. In the absence of stable supply, the scarcity of the resource leads to a significant rise in prices, with organizations attempting to acquire more than their fair share, always at the expense of others. This can lead to a situation where the most powerful or well-connected individuals or organizations are able to acquire the majority of resources, leaving the less fortunate with little to no access to the vital resource. To prevent such scenarios, {\em our goal is to increase the flow of the resource} to passive buyers, rather than allowing the distribution of scarce resources to be concentrated among the most active participants in the market. This can be achieved by creating a market for the resource, where buyers can purchase the resource at a fair price, or by implementing a rationing system where resources are distributed based on pre-established rules of fairness.

In summary, distribution crises are extreme situations where the availability of a vital resource is limited, and it is important to consider the ethical fairness of the distribution and the presence of a market to ensure an equitable distribution of resources. Such approach may be thought of as analogous to the basic strategy of \cite{DKA} which however studies a different problem, namely maximizing the potential of the marketplace itself to serve as a re-distributive tool.

\subsection{Related work}
Related work, particularly in the lengthy history of market design for efficiently allocating indivisible goods. 

Positioning amongst existing literature. I know there has been work studying the resale of pollution rights in carbon markets as well as distributing food bank allocations for instance. 

\subsection{Main idea}
\label{sub.mi}
For simplicity, we assume that there is only one commodity to be distributed. Our system is formed by a sequence of markets happening sequentially over discrete time.  Each market has two parts:
1. Sellers announce the supply for the critical commodity and buyers announce the demand for the commodity.
On the basis of this input, the system assigns, according to pre-agreed rules of fairness (see Section \ref{sec.fair}) to each buyer a fair amount of {\em rights to purchase the commodity}.
2. In each market of the sequence, both the critical commodity and the rights are traded. There is only one limitation: at the end of each market, each buyer must have at least as big amount of rights as of the commodity. Uncoupled rights disappear in the end of each market. 

The idea is that some (active) buyers want to buy more of the good right away, so according to the rules of the market, they can buy from hesitant (passive) buyers an amount of rights assigned to them. With this money saved, even these passive buyers can buy the commodity in next markets, because the rights are recalculated before each market, and thus renewed.

%Buyers can therefore determine their individual benefit when investing and purchasing goods themselves according to their current needs and on the basis of the calculation of the benefit/price ratio, specifically for each market. 
%There are three basic types of buyers. (1) The buyer buys exactly as much of the good on the market as it has assigned rights. (2) The buyer (active) buys more goods than it has assigned rights, and it has to buy additional rights from other market participants. (3) The buyer (passive) buys less goods than it has assigned rights and sells its remaining rights.


%Active buyers may choose to increase the volume of purchases by purchasing rights from other participants and thus invest more. Passive buyers who, for whatever reason, consider that they do not want or do not need to use the assigned rights to purchase goods in a given market, will receive funds from the sale of their rights, which they can then use according to their needs, either to purchase the rights from other buyers in the following market and thus purchase a larger quantity of scarce goods at a later date, or they can use them to pay for the goods purchased according to their assigned rights, which means that the final price they pay for the purchased goods will be lower for them.



%{\em In this way, active buyers get more of the commodity, much as they would get on the free market.But at the same time, they will pay for the rights to passive buyers, thereby expanding the flow of money in the market, and passive buyers will effectively get extra funds to buy the commodity or rights in the next market following the current one.In each market, buyers will get new rights to buy the commodities on a fair basis and independently of the market that has just ended. We will argue that he resulting benefit for all market participants, i.e. participating buyers and suppliers, increases by widening of the flow of money and critical goods and is higher than by trading on the open market.}

%\medskip
%Our suggested way of dealing with the distribution of scarce material in times of crisis therefore admits a strategy for specific market participants so that the profit of one group (e.g. more of purchased goods) does not mean a loss for the other group, but on the contrary, it also brings them a profit (e.g. financial profit from the sale of the rights). The resulting benefit for all market participants, i.e. participating buyers and suppliers, increases by the widening of the flow of money and critical goods and is higher than by trading on the open market.

%Active buyers, instead of the classic bidding process, have to buy 'rights to buy' in addition to the commodity, when the quantity requested exceeds the fair part.As a result, they will pay the final amount which is increased by the purchase price of these rights. The main idea of our solution is that this increase will be given to passive buyers and will help them to buy either the fair part of the commodity or the rights to purchase more than fair amount in the next market. Summarizing,Active buyers buy, without delay, more than the fair amount (they will pay for it).Passive buyers are allowed to buy a quantity of the commodity that they would not get on the free market, albeit with some delay.Suppliers will sell the goods at the higher price to a wider group of buyers and stay on the market.



\subsection{Frustration and Willingness to Pay}
\label{sub.fru}
We need to introduce some measures indicating how successful the proposed hybrid mechanism is towards our goal of widening the flow of the critical commodity in the time of a distribution crisis. 
For a single market, we define the {\em frustration} of a buyer $b$ as the ratio $0\leq a/r\leq 1$ where $r$ is the amount of the rights potentially assigned to $b$ and $a$ is the difference between $r$ and the amount of the good purchased by $b$, if this is at least zero, and it is defined to be zero otherwise.
We note that the notion of frustration extends to normal times without crises and to the unrestricted free market with the critical commodity. In normal times, the amount of assigned rights is equal to the demand and moreover $b$ can buy all the goods it demands. Hence, its frustration is zero. Our concept of {\em frustration} is somewhat similar to  the {\em deprivation cost} of \cite{HPJ}.

Our aim is to show that in a sequence of markets of our system, {\em the frustration of each buyer becomes smaller than it would be in the free market}. In order for that to happen it is needed that the frustrated buyers increase their {\em willingness to pay} (formally introduced in Definition \ref{def.ww}).  Our proposed mechanism changes the willingness to pay by trading the assigned rights.

\subsection{Coalition Proofness} \todo{text then pointer to subsection} 

\subsection{Main Contribution} 

%\todo {REWRITE AS LAST THING. A main contribution as stated in the paper is that the proposed algorithmmore “fairly” allocates the scarce good, but this definition is not made precise inthe paper.}


We consider the question of how to allocate a good that is over-demanded in a  multi-round scenario which we call a {\em distribution crisis}, in order to improve the fairness of the free market allocation. 

This is by itself an important subject of economic interest. We believe that our construction, in particular introducing rights to purchase,
separating rights and goods and trading them separately may be useful in other fairness contexts as well.

A distribution crisis for a commodity which needs to be supplied regularly is typically preceded by significant changes in demand and/or supply, causing a sudden change of the market. Modelling these early stages is a growing research area [???], however typically requires non-trivial assumptions about the nature of the crisis. 

Final rounds of a distribution crisis are also very complex to model and analyse since an optimal outcome of a participant for the terminal segment of a crisis does not necessarily decompose into his optimal outcomes in each round; the participants strategize when a termination of a crisis becomes apparent.

We instead choose to model the middle of the multi-round distribution crisis, where the supply and demand is relatively stable and the participants aim the optimal outcome of each round. We call each round a {\em Market}.

We further simplify by having only one type of scarce resource called {\it Good}. 

%\todo{ Assuming that the central authority managing the market is able to enforce truthfulness for buyers’ reported demands also seems like a strong assumption that weakens the results. There is also the assumption (as far as I can tell) that the number of goods in each round is constant and known to all buyers which drastically simplifies the setting.}

Our multi-round trading environment, which we call {\em Crisis}, is formally introduced in Section \ref{sec.def}.

First step in  is to have a benchmark "fair" allocation given the needs of the buyers and the supply of the suppliers. We go into more detail on what ``fair" means in Section \ref{sec.fair}.

The second step of our solution is introduction of a trading environment which is meant to increase fair allocation of Good among buyers.  We accomplish this by introducing a new tradable commodity which we call {\it Right}: it represents right to buy Good and it is distributed in the beginning of each round according to the benchmark allocation. Without the Right, our solution reduces to the multi-round free market for the Good.

A key new idea is, in each round, to trade separately allocated amount of Right and available amount of Good.  Agents who have the rights to an amount of Good but whose per-unit utility is low can sell their rights to others, raising funds to purchase Good in future rounds.

In Section \ref{sec.alg}, we describe a polynomial auction-based algorithm called {\em Couple} and show in Theorem \ref{thm.mmain} that for a practically non-restrictive choice of parameters it outputs an approximate optimal market clearing solution for the Crisis. 

In the remaining part of the paper, starting with Theorem \ref{thm.wp}, we further assume that the amount of Good in each round as well as the utilities of traders are constant. This is a realistic assumption for the middle of a distribution crisis.

We first show that in Theorem \ref{thm.wp} that the outcome of the Couple decreases the frustration of the participants to at most $1/2$. This is a significant improvement to the worst case frustration $1$ for the free market.

In later sections, we introduce and analyse a realistic double-sided mechanism for Crisis.

It is convenient to change the setting and define this mechanism as a {\em sequential game} rather than a multi-round trading environment.

Informally, an interaction between buyers and sellers is as follows. First, each seller offers some amount of Good he has for sale for some price. Based on the total offered volume of Good and the Demand of buyers, a central {\it fairness mechanism} then assigns buyers with Right. In the second stage, the buyers offer some amount of Right for sale for a fixed price. Given offers for both Right and Good, the buyers then declare maximum volume and price they are willing to pay for both. A {\it market mechanism} then clears the bids. 

We show that 
the introduced mechanism approximates the fair benchmark allocation at an equilibrium of behavior.


==> common/import.tex <==
\usepackage[in]{fullpage}
\usepackage[T1]{fontenc}
\usepackage{graphicx}
\usepackage{hyperref}
\usepackage{color}
\renewcommand\UrlFont{\color{blue}\rmfamily}

\usepackage{csquotes}
\usepackage{amsmath}
% \usepackage{amsthm}
% \usepackage{amssymb}
\usepackage{mathtools}
\usepackage{multicol}

% %%%%%%%% ALGS
\usepackage[ruled, noend]{algorithm2e} % For algorithms
% \renewcommand{\algorithmcfname}{ALGORITHM}
% \SetAlFnt{\small}
% \SetAlCapFnt{\small}
% \SetAlCapNameFnt{\small}
% \SetAlCapHSkip{0pt}
% \IncMargin{-\parindent}
\usepackage{algpseudocode}
\usepackage{caption}
\usepackage{subcaption}

